Addressing Data Annotation Challenges in Multiple Sensors: A Solution for Scania Collected Datasets

Data annotation in autonomous vehicles is a critical step in the development of Deep Neural Network (DNN) based models or the performance evaluation of the perception system. This often takes the form of adding 3D bounding boxes on time-sequential and registered series of point-sets captured from active sensors like Light Detection and Ranging (LiDAR) and Radio Detection and Ranging (RADAR). When annotating multiple active sensors, there is a need to motion compensate and translate the points to a consistent coordinate frame and timestamp respectively. However, highly dynamic objects pose a unique challenge, as they can appear at different timestamps in each sensor's data. Without knowing the speed of the objects, their position appears to be different in different sensor outputs. Thus, even after motion compensation, highly dynamic objects are not matched from multiple sensors in the same frame, and human annotators struggle to add unique bounding boxes that capture all objects. This article focuses on addressing this challenge, primarily within the context of Scania collected datasets. The proposed solution takes a track of an annotated object as input and uses the Moving Horizon Estimation (MHE) to robustly estimate its speed. The estimated speed profile is utilized to correct the position of the annotated box and add boxes to object clusters missed by the original annotation.

==> sections/EXPERIMENTS/comparison_to_baseline.tex <==
% \subsection{Runtime}
\subsection{Comparison to Baseline}     
\label{subsec:comparison_baseline}

\input{tables/Baseline_comparison}

%A detailed 
A comparison between our algorithms and their respective baselines as a function of the range is shown in~\Cref{tab:commparison_baseline}. To guarantee a fair comparison, we re-train the baseline networks for six epochs using \gls{cbgs}, which we denote by $*$. We also provide the performance reported by the authors of the baseline for completeness, denoted by $\dagger$. For \gls{fsd}, we reduce the minimum points for clustering from two to one, to enable clustering at long range. It's observed that using \gls{cbgs} seems to slightly benefit long range performance. For both baselines, a consistent improvement across ranges can be attributed to the respective range experts specializing in their domain. Nevertheless, very little improvement is observed in 200-250\si{m} range, perhaps because labels in this range constitute only 0.3\% of the dataset, as shown in \cref{fig:Statistics_dataset}. Our results underscore the substantial room for improvement within the current state-of-the-art for long-range 3D detection. 
%Our results also demonstrate that there is a large scope for improvement in current state-of-the-art.

%To guarantee a fair comparison, we re-train the baseline network for the same number of epochs with MVP and range weights (our contribution) and without them (fair comparison). In both cases we use CBGS \cite{zhu2019class} while training. We also provide the performance reported by the authors of the baseline for completeness. 


%By increasing the training time, a slight improvement in performance is observed, however, the MVP and range weighting clearly boost the performance. This improvement is observed for most\footnote{In the 0-50~\si{m} range, the additional training epochs with \gls{cbgs} result in a degrade in performance, making the original \gls{fsd}v2$\dagger$ algorithm the most optimal at this range.}  distances, but it is especially beneficial for objects above 50~\si{m} which are traditionally disregarded by most short range algorithms.



==> sections/EXPERIMENTS/effect_2d_backbone.tex <==
% \subsection{Ablation Studies}   \label{subsec:ablation_studies} 
\subsection{Effect of image segmentation}   \label{subsec:2d_backbone} 
%\textbf{Effect of 2D backbone:}
%We analyze the effect of the image segmentation quality on the performance 
% In order to analyze the robustness of the proposed approach to image segmentation, 
To analyze the impact of image segmentation backbone on the performance of our proposed approach, 
we replace HTC~\cite{chen2019hybrid} (default 2D segmentor) with Mask RCNN~\cite{he2017mask},  another well known image segmentor.
%, albeit with a lower mask and box mAP. 
As shown in \Cref{table:effect_2d_backbone}, our finetuned RangeFSD with Mask RCNN gives similar results to HTC, demonstrating robustness to the 2D segmentor employed. On the other hand, the significantly higher mask and box mAP for HTC indicates that while both the segmentors seem to detect mid range objects equally well, HTC could be better at detecting small objects.
%, including those at long range. 
%Some of these could well be at long range and out of reach for current \gls{lidar}s, in which case a \gls{lidar}-only detector cannot detect them.
Some of these small objects could very well be at large distances, outside the reach of \gls{lidar} points, making it impossible for a \gls{lidar}-only detector to detect them.
\input{tables/Ablation_img_backbone}



==> sections/EXPERIMENTS/performance_breakdown.tex <==
\subsection{Performance Breakdown}  \label{subsec:performance_breakdown}
Our contribution can be divided into two components: implementation of \gls{mvp} and range experts. In order to assess the impact of each component on our final state-of-the art algorithms, a detailed performance breakdown, shown in \Cref{tab:perf_breakdown}, is performed. 

\input{tables/Performance_breakdown}

The impact of \gls{mvp}
% with and without finetuning 
is studied independently for the \gls{fsd} and RangeFSD. 
% The finetuning of \gls{mvp} proves to be crucial in both cases, where a drop in performance is observed when implementing the \gls{mvp} without finetuning.
It was observed that finetuning after adding virtual points is crucial for both the cases. A significant drop in performance is observed when applying \gls{mvp} without finetuning.
This drop could be explained by a shift in point distribution caused by \gls{mvp}. The \gls{lidar} pre-segmentor, used by both baselines, is negatively affected by this shift and hence needs to be finetuned. Overall, \gls{mvp} contributes to about 1.7\% increase in \gls{map}, whereas the range expert contributes about 0.4\% \gls{map}. Although a higher boost in performance arises from \gls{mvp}, a combination of \gls{mvp} and range experts is required to maximise the performance of \gls{fsd}. 

% The impact of MVP with and without finetuning is studied independently for the FSD and RangeFSD algorithms. The finetuning of MVP proves to be crucial in both cases, where a drop in performance is observed when implementing the MVP without finetuning. This drop can be attributed to a shift in point distribution caused by MVP.  
%The finetuned MVP implementation drastically improves the performance for both algorithms at all distances. Furthermore, for all tested configurations, RangeFSD performs better or than FSD for distances below 200 m. No improvement is observed for objects above 200 m. %Depending on the distance, the boost in performance arising from the range experts is between 0--40\% lower when combined with MVP than when applied alone. This indicates that, 
%The overall best performance is obtained when combining both MVP with finetuning and range experts. It is worth noting that, for distances below 150 m, the boost in performance from the range experts is up to 40\% lower when combined with MVP than when applied alone. This indicates a small correlation between the correctly classified objects between MVP and range experts at this distances. No correlation is observed for distances above 150 m. A higher boost in performance arises from implementing MVP, however, the combination of MVP and range experts is required to maximise the performance of the FSD algorithm.


==> sections/EXPERIMENTS/sota_comparison.tex <==
\subsection{State-of-the-art Comparison}    \label{subsec:sota}
% Points to cover here: fsdv2 with mvp and range weights gives best performance. although many categories improve,  
\input{tables/SOTA_comparison_without_dollar}

The comparison of different state-of-the art algorithms is shown in \Cref{table:sota_comparison}. Our algorithms, marked with $^{*}$, outperform their respective baselines, as well as all previous state-of-the-art methods.
The evaluation range is set to 0-200~\si{m} to enable a fair comparison to other methods.
%algorithms. Furthermore, RangeFSDv2 outperforms all previous \gls{lidar} based state-of-the-arts. 
Although improvements span across many classes, they are especially notable for 
%Notable improvements are observed for 
vulnerable road users (2-3\% for pedestrians, motorcyclist, bicyclist) and small objects (3-10\% for motorcycle, bicycle and construction cones). Equally interesting is the drop in performance for some classes, as compared to \gls{fsd}v2 baseline. 
%The reason for this gap can be attributed to the image segmentor generating the virtual points, specifically the dataset it's trained on,  As mentioned
This drop could be caused by the noise in the virtual point generation process, which in turn is caused by noisy masks generated by the 2D segmentor, for classes it is not trained on. 
%This drop can be attributed to the image segmentor generating the virtual points. 
As mentioned earlier, we use an off-the-shelf 2D segmentor (HTC~\cite{chen2019hybrid}) trained on the NuImages dataset. 
% which has 10 classes. 
We perform a one-to-one mapping between NuImage classes and their best match among the 26 classes in the \gls{av2} dataset. Inevitably, some classes not covered by this scheme don't improve (like box truck), or even get worse if mislabeled (eg. wheelchair, sign, stop sign etc.). 
%On the other hand, even though there is no explicit label for motorcyclists and bicyclists in NuImages, the segmentor probably detects them as pedestrians and correctly generates the virtual points. 
%%This underscores our design choice of omitting the semantic label from the virtual point feature, compared to original implementation of MVP~\cite{yin2021multimodal}. 


% \input{tables/Custom_Table_AP} % Not sure if this should go here

%\input{tables/Custom_Table_AR} % Not sure if this should go here

% \input{tables/Custom_Table_all_AR} % Not sure if this should go here

% \input{tables/Custom_Table_Experiments_AP}




==> sections/EXPERIMENTS/speed_plots_10-40/4BFCCD5D-3B39-4DE8-BB46-696D55F0B731.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={time (sec)},
xmajorgrids,
xmin=0, xmax=10,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Speed (m/s)},
ymajorgrids,
ymin=10, ymax=40,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0 20.4498762216466
0.1 20.4507055044172
0.2 20.4525255036302
0.3 20.4549858858171
0.4 20.4568146940589
0.5 20.4577662538073
0.6 20.4577545653734
0.7 20.4568989575321
0.8 20.4555156072152
0.9 20.4536823223833
1 20.4510313904608
1.1 20.4478812995496
1.2 20.4453615743268
1.3 20.4450335751616
1.4 20.4457222418622
1.5 20.4459188670447
1.6 20.4453258979015
1.7 20.4434700407626
1.8 20.4405159722041
1.9 20.4374964571825
2 20.4344940897706
2.1 20.4316253671016
2.2 20.4289702202227
2.3 20.4258999819205
2.4 20.4215186676638
2.5 20.4156985477101
2.6 20.4080159336197
2.7 20.3985433078127
2.8 20.3878489835177
2.9 20.3777172062348
3 20.3680784384135
3.1 20.3583072078572
3.2 20.3467912396201
3.3 20.333374178973
3.4 20.3203055336638
3.5 20.3083890007157
3.6 20.2978491499449
3.7 20.2885994984039
3.8 20.280567642558
3.9 20.2735217844652
4 20.2668366626852
4.1 20.260277926547
4.2 20.253688698539
4.3 20.2470827484021
4.4 20.2406502751248
4.5 20.2339382778079
4.6 20.2268746095914
4.7 20.2196026207224
4.8 20.2114741072611
4.9 20.2018199054106
5 20.1899874202743
5.1 20.1762304357072
5.2 20.160705004959
5.3 20.1437954796122
5.4 20.1277668978775
5.5 20.1132337623269
5.6 20.1002432463329
5.7 20.0885029042566
5.8 20.0776924028845
5.9 20.0672240752621
6 20.0569118916739
6.1 20.0467510340564
6.2 20.0369319380833
6.3 20.026984747553
6.4 20.0169102642914
6.5 20.0065629714905
6.6 19.99572799669
6.7 19.9843156082997
6.8 19.9723593142185
6.9 19.9603876879742
7 19.9489854546561
7.1 19.9381865924167
7.2 19.9277086884557
7.3 19.9169812107196
7.4 19.9062634685108
7.5 19.8950351553709
7.6 19.8831033335048
7.7 19.8706976504507
7.8 19.8574844391847
7.9 19.8437703709571
8 19.8299032915021
8.1 19.8153950102425
8.2 19.8001340337515
8.3 19.7847129132404
8.4 19.7716267534977
8.5 19.7614896279639
8.6 19.7541141898482
8.7 19.7489590724135
8.8 19.7451186866824
8.9 19.7423155125339
9 19.7400061199495
9.1 19.7374416664309
9.2 19.734923630639
9.3 19.7333584251729
9.4 19.7327297696866
9.5 19.7326350230567
9.6 19.7325804838289
};
\addlegendentry{MHE}
\addplot [semithick, darkorange25512714]
table {%
0 20.3229451179504
0.1 20.3006315231323
0.2 20.3006315231323
0.3 20.2968072891235
0.4 20.6198644638062
0.5 20.5640006065369
0.6 20.5661177635193
0.7 20.5753469467163
0.8 20.455858707428
0.9 20.4601120948792
1 20.5666279792786
1.1 20.5498290061951
1.2 20.4277467727661
1.3 19.9656701087952
1.4 20.3286409378052
1.5 20.6374287605286
1.6 20.5268001556396
1.7 20.6461191177368
1.8 20.6331181526184
1.9 20.3376603126526
2 20.4433298110962
2.1 20.4340934753418
2.2 20.3414607048035
2.3 20.4391121864319
2.4 20.6343865394592
2.5 20.5257439613342
2.6 20.6432056427002
2.7 20.6486487388611
2.8 20.6486678123474
2.9 20.1436305046082
3 20.2751159667969
3.1 20.2695608139038
3.2 20.6640553474426
3.3 20.7815027236938
3.4 20.1536726951599
3.5 20.1537489891052
3.6 20.149974822998
3.7 20.1628994941711
3.8 20.1498961448669
3.9 20.1400566101074
4 20.2710437774658
4.1 20.2710819244385
4.2 20.2804112434387
4.3 20.2766609191895
4.4 20.1717615127563
4.5 20.3053164482117
4.6 20.3015923500061
4.7 20.171365737915
4.8 20.3066325187683
4.9 20.3685998916626
5 20.5041480064392
5.1 20.3781366348267
5.2 20.3774118423462
5.3 20.4976177215576
5.4 19.8998034000397
5.5 19.923107624054
5.6 19.9279522895813
5.7 19.9643337726593
5.8 19.9692118167877
5.9 20.0809478759766
6 20.0728964805603
6.1 20.0647902488708
6.2 19.9454724788666
6.3 20.0985956192017
6.4 20.019063949585
6.5 20.0372815132141
6.6 20.0610876083374
6.7 20.0625371932983
6.8 20.0809478759766
6.9 19.9745631217957
7 19.8461067676544
7.1 19.8551523685455
7.2 19.8792040348053
7.3 20.0316214561462
7.4 19.8347687721252
7.5 19.9795985221863
7.6 20.0018215179443
7.7 19.8678576946259
7.8 20.0166988372803
7.9 19.9124646186829
8 19.7781753540039
8.1 19.9308741092682
8.2 19.9589836597443
8.3 20.0034236907959
8.4 19.3607842922211
8.5 19.3960702419281
8.6 19.4499826431274
8.7 19.4942772388458
8.8 19.6832919120789
8.9 19.618399143219
9 19.6758997440338
9.1 19.8744249343872
9.2 19.7967302799225
9.3 19.5468497276306
9.4 19.6009123325348
9.5 19.6713078022003
9.6 19.8571908473969
};
\addlegendentry{Naive}
\end{axis}

\end{tikzpicture}


==> sections/EXPERIMENTS/speed_plots_10-40/6E605C66-14FF-4F62-87CD-7E0A2422C7AD.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={time (sec)},
xmajorgrids,
xmin=0, xmax=10,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Speed (m/s)},
ymajorgrids,
ymin=10, ymax=40,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0 20.1769414683517
0.1 20.1665957654071
0.2 20.1431463356251
0.3 20.1087506756272
0.4 20.0728319061697
0.5 20.0390760578732
0.6 20.0082824500756
0.7 19.9806907983224
0.8 19.9563878981525
0.9 19.9348721682812
1 19.9153438194472
1.1 19.8976794859497
1.2 19.8822745820258
1.3 19.8690037234332
1.4 19.8582066399404
1.5 19.8500453409715
1.6 19.8442172906001
1.7 19.840014733738
1.8 19.8370146616863
1.9 19.8347520189544
2 19.8328601840433
2.1 19.8314255841951
2.2 19.8308712833601
2.3 19.8315457622516
2.4 19.8353005928434
2.5 19.8430500247682
2.6 19.8546105434967
2.7 19.8696552429244
2.8 19.8871105808748
2.9 19.9039946118161
3 19.9188183597231
3.1 19.9312423783121
3.2 19.9416963504383
3.3 19.9506112283154
3.4 19.9597802963096
3.5 19.9699493348795
3.6 19.9814004700558
3.7 19.9940577514415
3.8 20.0076150939978
3.9 20.0209068619631
4 20.0330661506037
4.1 20.0439024737628
4.2 20.0534374461228
4.3 20.0620085025638
4.4 20.0704325704857
4.5 20.0786030105084
4.6 20.0867372092346
4.7 20.0953441791989
4.8 20.1044284572518
4.9 20.1147650273769
5 20.1261973155512
5.1 20.1388511563265
5.2 20.1526514792699
5.3 20.1671584691098
5.4 20.182111734513
5.5 20.1973397396286
5.6 20.2127537268371
5.7 20.2281424599491
5.8 20.243288008004
5.9 20.2575525651643
6 20.2708825273478
6.1 20.2834724446612
6.2 20.2957432990037
6.3 20.307491684691
6.4 20.319070487607
6.5 20.3305860772076
6.6 20.3420142497453
6.7 20.3533680293323
6.8 20.3645793683162
6.9 20.3755444829903
7 20.3867414796733
7.1 20.3982831096494
7.2 20.4100062426433
7.3 20.4213949633655
7.4 20.4325366874725
7.5 20.4429674368807
7.6 20.4526403566279
7.7 20.461947672211
7.8 20.470671962576
7.9 20.4790981254641
8 20.4876635765059
8.1 20.4959626904166
8.2 20.503805087589
8.3 20.5112336785294
8.4 20.518945615087
8.5 20.5270030966704
8.6 20.5351504287515
8.7 20.5430107988194
8.8 20.5500876071967
8.9 20.5570315978405
9 20.5636484915298
9.1 20.5692107719865
9.2 20.5736479738223
9.3 20.576645806034
9.4 20.5779977564454
9.5 20.577903590977
9.6 20.5778492215325
};
\addlegendentry{MHE}
\addplot [semithick, darkorange25512714]
table {%
0 21.9890475273132
0.1 21.9667530059814
0.2 21.9667410850525
0.3 21.9629192352295
0.4 19.6846008300781
0.5 19.5698523521423
0.6 19.6764135360718
0.7 19.6856641769409
0.8 19.560239315033
0.9 19.6514248847961
1 19.7638463973999
1.1 19.7469174861908
1.2 19.6196854114532
1.3 19.7295498847961
1.4 19.6237182617188
1.5 19.570837020874
1.6 19.596825838089
1.7 19.7215569019318
1.8 19.7084856033325
1.9 19.7584974765778
2 19.8480355739594
2.1 19.8388183116913
2.2 19.7386240959167
2.3 19.8540806770325
2.4 19.4312727451324
2.5 19.3165409564972
2.6 19.44011926651
2.7 19.4455409049988
2.8 19.4455409049988
2.9 20.0918340682983
3 20.2283501625061
3.1 20.2229189872742
3.2 20.1145172119141
3.3 20.2372717857361
3.4 19.8212218284607
3.5 19.8212206363678
3.6 19.8174679279327
3.7 19.8305010795593
3.8 19.8173916339874
3.9 20.0615572929382
4 20.1961398124695
4.1 20.1961398124695
4.2 20.2054762840271
4.3 20.2014493942261
4.4 19.9907231330872
4.5 20.1263284683228
4.6 20.1223349571228
4.7 19.9912059307098
4.8 20.1274752616882
4.9 19.8883128166199
5 20.026261806488
5.1 19.9891245365143
5.2 19.9887454509735
5.3 20.1102542877197
5.4 20.1402950286865
5.5 20.1638841629028
5.6 20.1690053939819
5.7 20.2056646347046
5.8 20.2106666564941
5.9 20.3867769241333
6 20.3790855407715
6.1 20.3711938858032
6.2 20.2520203590393
6.3 20.4057240486145
6.4 20.2937698364258
6.5 20.3125882148743
6.6 20.3363609313965
6.7 20.3383874893188
6.8 20.3570938110352
6.9 20.4427409172058
7 20.3140687942505
7.1 20.3233098983765
7.2 20.3473472595215
7.3 20.4998302459717
7.4 20.3879523277283
7.5 20.5347371101379
7.6 20.5569815635681
7.7 20.4218602180481
7.8 20.5718517303467
7.9 20.5164337158203
8 20.3836727142334
8.1 20.5348539352417
8.2 20.5626368522644
8.3 20.6072354316711
8.4 20.4169201850891
8.5 20.4519033432007
8.6 20.5059623718262
8.7 20.5504083633423
8.8 20.7394528388977
8.9 20.4826784133911
9 20.5402207374573
9.1 20.7388734817505
9.2 20.661039352417
9.3 20.7277250289917
9.4 20.7816314697266
9.5 20.8522725105286
9.6 21.0379409790039
};
\addlegendentry{Naive}
\end{axis}

\end{tikzpicture}


==> sections/EXPERIMENTS/speed_plots_10-40/B4F3168E-25B4-4906-8E00-FEB72582FAED.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={time (sec)},
xmajorgrids,
xmin=0, xmax=10,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Speed (m/s)},
ymajorgrids,
ymin=10, ymax=40,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0 25.6084679138508
0.1 25.6094041967731
0.2 25.6116773397279
0.3 25.6151576232195
0.4 25.6191299666102
0.5 25.6233245714569
0.6 25.6276862817905
0.7 25.6320713228622
0.8 25.6363406685305
0.9 25.6403256037506
1 25.6439655647448
1.1 25.6473329173021
1.2 25.650574468172
1.3 25.6538446748262
1.4 25.6572293398491
1.5 25.6607834292203
1.6 25.6644415784891
1.7 25.668447722137
1.8 25.6728446898406
1.9 25.678263738935
2 25.6848791326361
2.1 25.6927945602685
2.2 25.7020091708541
2.3 25.7125221763993
2.4 25.7245145306456
2.5 25.7379942907816
2.6 25.7530058325905
2.7 25.7695277748385
2.8 25.787319648385
2.9 25.8055820798725
3 25.823668413919
3.1 25.8438474136092
3.2 25.864990211607
3.3 25.8869482195731
3.4 25.9104924894358
3.5 25.9360196378432
3.6 25.9637800931396
3.7 25.9938485375083
3.8 26.0262379382994
3.9 26.0603851983994
4 26.0961475819794
4.1 26.1338535613151
4.2 26.1737910332307
4.3 26.2159540991204
4.4 26.2600829173214
4.5 26.3043772123665
4.6 26.3433990841752
4.7 26.3622151949471
4.8 26.3212477190565
4.9 26.2612495191405
5 26.1973877287625
5.1 26.1350893064664
5.2 26.0761551721348
5.3 26.0212284230323
5.4 25.9711034313251
5.5 25.9257816801888
5.6 25.8848541635923
5.7 25.8479117643181
5.8 25.8144419318816
5.9 25.7840584654671
6 25.7564333758452
6.1 25.7311995373523
6.2 25.7080456220988
6.3 25.6867018031693
6.4 25.6670257798495
6.5 25.6487028019002
6.6 25.6314861396275
6.7 25.6153048116259
6.8 25.5999713194262
6.9 25.5852958407206
7 25.5711265277959
7.1 25.5572843947664
7.2 25.5436785440755
7.3 25.5302836642256
7.4 25.517415136358
7.5 25.5051807959526
7.6 25.4934842864395
7.7 25.4821241906192
7.8 25.4707520169498
7.9 25.4586454550795
8 25.4454062007687
8.1 25.4307552937341
8.2 25.4141410799955
8.3 25.3951080637209
8.4 25.3728605997019
8.5 25.3468630129255
8.6 25.3169749491917
8.7 25.2837284634814
8.8 25.2492420101192
8.9 25.2197246179845
9 25.1972739280935
9.1 25.1823136206492
9.2 25.1743064540085
9.3 25.1718550438089
9.4 25.1712233945417
9.5 25.1711123410585
9.6 25.171048239701
};
\addlegendentry{MHE}
\addplot [semithick, darkorange25512714]
table {%
0 25.4089665412903
0.1 25.463445186615
0.2 25.4237604141235
0.3 25.4337024688721
0.4 25.6101965904236
0.5 25.6228756904602
0.6 25.5885767936707
0.7 25.6413888931274
0.8 25.6067109107971
0.9 25.6798052787781
1 25.6446027755737
1.1 25.6401991844177
1.2 25.6576442718506
1.3 25.6532144546509
1.4 25.6582927703857
1.5 25.6510782241821
1.6 25.7024717330933
1.7 25.6212735176086
1.8 25.6801414489746
1.9 25.5085277557373
2 25.5563545227051
2.1 25.5639410018921
2.2 25.5663657188416
2.3 25.5863308906555
2.4 25.5489444732666
2.5 25.5687952041626
2.6 25.5692887306213
2.7 25.5944299697876
2.8 25.5950736999512
2.9 25.7541871070862
3 26.1189293861389
3.1 25.2612662315369
3.2 25.8300280570984
3.3 25.8804535865784
3.4 25.691020488739
3.5 25.7054924964905
3.6 25.7075357437134
3.7 25.7194399833679
3.8 25.7037234306335
3.9 25.8904337882996
4 25.9402084350586
4.1 25.9086942672729
4.2 25.8812713623047
4.3 25.9302401542664
4.4 25.8720231056213
4.5 25.8782029151917
4.6 25.8938789367676
4.7 25.9030032157898
4.8 40.3767108917236
4.9 25.6689763069153
5 25.6654691696167
5.1 25.6838226318359
5.2 25.6833243370056
5.3 25.7017636299133
5.4 25.4711556434631
5.5 25.451557636261
5.6 25.4888701438904
5.7 25.4665899276733
5.8 25.5130362510681
5.9 25.5080008506775
6 25.5073094367981
6.1 25.526225566864
6.2 25.5256485939026
6.3 25.5411982536316
6.4 25.4953384399414
6.5 25.5380725860596
6.6 25.5474328994751
6.7 25.5121660232544
6.8 25.5217719078064
6.9 25.5319166183472
7 25.5288624763489
7.1 25.5451035499573
7.2 25.5424070358276
7.3 25.552179813385
7.4 25.4534959793091
7.5 25.4217791557312
7.6 25.4344129562378
7.7 25.4380536079407
7.8 25.4473519325256
7.9 25.5777764320374
8 25.5872344970703
8.1 25.5588173866272
8.2 25.6344175338745
8.3 25.6187677383423
8.4 25.7399988174438
8.5 25.7869172096252
8.6 25.8033180236816
8.7 25.810124874115
8.8 25.8201289176941
8.9 24.3453478813171
9 24.3497490882874
9.1 24.3567180633545
9.2 24.4049453735352
9.3 24.3842887878418
9.4 25.2332973480225
9.5 25.203104019165
9.6 25.2227163314819
};
\addlegendentry{Naive}
\end{axis}

\end{tikzpicture}


==> sections/EXPERIMENTS/speed_plots_10-40/D61F7DC7-289B-490D-96F3-9D47ECF85A16.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={time (sec)},
xmajorgrids,
xmin=0, xmax=10,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Speed (m/s)},
ymajorgrids,
ymin=10, ymax=40,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0 12.6507820960786
0.1 12.6613025608338
0.2 12.6863081624062
0.3 12.7268833185599
0.4 12.7822639497296
0.5 12.8525456578148
0.6 12.9378774641921
0.7 13.0383248277184
0.8 13.152980816094
0.9 13.2785537189247
1 13.414267886241
1.1 13.5604111738738
1.2 13.7173101448841
1.3 13.883998473888
1.4 14.0555499815617
1.5 14.2308690770581
1.6 14.410165951287
1.7 14.5932131141826
1.8 14.7775057643944
1.9 14.9543964671142
2 15.1215887496748
2.1 15.2793200921773
2.2 15.4288079649247
2.3 15.5717000236849
2.4 15.7106074174208
2.5 15.8471229646218
2.6 15.982534994791
2.7 16.1177360728308
2.8 16.2522425065543
2.9 16.3827398158624
3 16.5088376269833
3.1 16.6309030080818
3.2 16.7496247561611
3.3 16.8654983177642
3.4 16.9778568279177
3.5 17.0871670011625
3.6 17.1943091213796
3.7 17.2998901415937
3.8 17.4041646969923
3.9 17.5057485745862
4 17.604802360743
4.1 17.7017693403822
4.2 17.7968192512046
4.3 17.8887000287644
4.4 17.9728266101808
4.5 18.0478076503969
4.6 18.1135214894055
4.7 18.1700336094022
4.8 18.2169696796573
4.9 18.2524700932884
5 18.2759663238217
5.1 18.2873482641499
5.2 18.2865004244685
5.3 18.2730194057615
5.4 18.2457262029412
5.5 18.2042963594822
5.6 18.148941326402
5.7 18.0810336018439
5.8 18.0052472358695
5.9 17.9345177503072
6 17.8731871840919
6.1 17.8220012323254
6.2 17.779366667764
6.3 17.7406241783026
6.4 17.6935831183141
6.5 17.6333181380907
6.6 17.5577597197477
6.7 17.4665009248356
6.8 17.3606996310173
6.9 17.2450940495073
7 17.1208684265062
7.1 16.9879780514535
7.2 16.8463401677293
7.3 16.6968483373613
7.4 16.5437269482293
7.5 16.3879018700336
7.6 16.2292233846334
7.7 16.0675342233996
7.8 15.9036945104943
7.9 15.7416929956936
8 15.5824123964643
8.1 15.4256090611134
8.2 15.2712644710282
8.3 15.1204768046259
8.4 14.9777075634121
8.5 14.8441763017559
8.6 14.7200951526869
8.7 14.6056153943816
8.8 14.5018130890918
8.9 14.4121676368871
9 14.3378377962746
9.1 14.2791281401185
9.2 14.2361245225066
9.3 14.2088878037869
9.4 14.1971355112046
9.5 14.1970628179075
9.6 14.1970197840389
};
\addlegendentry{MHE}
\addplot [semithick, darkorange25512714]
table {%
0 10.8847212791443
0.1 10.9448206424713
0.2 10.9255504608154
0.3 10.9454822540283
0.4 11.3320231437683
0.5 11.3011384010315
0.6 11.331775188446
0.7 11.3417565822601
0.8 11.3517332077026
0.9 12.317156791687
1 12.3371160030365
1.1 12.3470962047577
1.2 12.3570466041565
1.3 12.3562896251678
1.4 13.7993490695953
1.5 13.8301146030426
1.6 13.8079071044922
1.7 13.8174974918365
1.8 13.8481962680817
1.9 16.1399364471436
2 16.1819291114807
2.1 16.181173324585
2.2 16.1484456062317
2.3 16.1802363395691
2.4 15.8683466911316
2.5 15.9094703197479
2.6 15.9094703197479
2.7 15.8761262893677
2.8 15.9085786342621
2.9 16.9417238235474
3 16.8989777565002
3.1 16.9308817386627
3.2 16.931654214859
3.3 16.9209134578705
3.4 17.3289382457733
3.5 17.3290145397186
3.6 17.2849345207214
3.7 17.3074185848236
3.8 17.2647738456726
3.9 17.8247165679932
4 17.7813017368317
4.1 17.7939581871033
4.2 17.7505350112915
4.3 17.783180475235
4.4 18.9886152744293
4.5 19.0126836299896
4.6 19.0027678012848
4.7 18.9918720722198
4.8 18.9819180965424
4.9 19.4920563697815
5 19.4931519031525
5.1 19.4921314716339
5.2 19.4832527637482
5.3 19.482079744339
5.4 19.7481727600098
5.5 19.7145569324493
5.6 19.7156620025635
5.7 19.7271645069122
5.8 19.695440530777
5.9 16.6378664970398
6 16.6378676891327
6.1 16.6278910636902
6.2 16.6592621803284
6.3 16.6386294364929
6.4 19.2915034294128
6.5 19.3014812469482
6.6 19.3226647377014
6.7 19.2813766002655
6.8 19.27241563797
6.9 17.9814827442169
7 17.9825723171234
7.1 17.9823434352875
7.2 17.9626798629761
7.3 17.9615128040314
7.4 16.7274105548859
7.5 16.6974854469299
7.6 16.6677892208099
7.7 16.6268634796143
7.8 16.597090959549
7.9 15.4105567932129
8 15.3600001335144
8.1 15.3570985794067
8.2 15.2901077270508
8.3 15.2494585514069
8.4 13.9927065372467
8.5 13.9529085159302
8.6 13.8934051990509
8.7 13.8524436950684
8.8 13.7809872627258
8.9 12.8576397895813
9 12.7982914447784
9.1 12.75723695755
9.2 12.7078855037689
9.3 12.6240026950836
9.4 12.307094335556
9.5 12.2449731826782
9.6 12.2055172920227
};
\addlegendentry{Naive}
\end{axis}

\end{tikzpicture}


==> sections/EXPERIMENTS/speed_plots_10-40/FE65FF93-A390-4FDA-A30E-7ECB649C971E.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={time (sec)},
xmajorgrids,
xmin=0, xmax=10,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Speed (m/s)},
ymajorgrids,
ymin=10, ymax=40,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0 30.1255188896752
0.1 30.1300353407321
0.2 30.1406130264684
0.3 30.1572049359939
0.4 30.1786478595219
0.5 30.2046224845787
0.6 30.2349671435926
0.7 30.2698776887905
0.8 30.3095380935017
0.9 30.3535919870932
1 30.4017099288114
1.1 30.4532129716726
1.2 30.5064603487044
1.3 30.5562262697634
1.4 30.5877291609422
1.5 30.5960021956223
1.6 30.5795262051078
1.7 30.5391735405896
1.8 30.4793603932081
1.9 30.4134402466963
2 30.3463980635791
2.1 30.2801431961371
2.2 30.2159003361899
2.3 30.1557108720444
2.4 30.1052945995229
2.5 30.0658059914637
2.6 30.0350806954668
2.7 30.0120050140672
2.8 29.9953534316293
2.9 29.9829865342702
3 29.9736502627567
3.1 29.9668020501834
3.2 29.9624506875125
3.3 29.9602318601233
3.4 29.9598643068033
3.5 29.9613610608356
3.6 29.964560566391
3.7 29.9693343095868
3.8 29.9748584576463
3.9 29.9786528503995
4 29.9795381222284
4.1 29.9770123014577
4.2 29.9706903080455
4.3 29.9606444216789
4.4 29.9476093961343
4.5 29.9318668010739
4.6 29.9133073774225
4.7 29.891801093898
4.8 29.8667951938062
4.9 29.8380832572887
5 29.8051523581953
5.1 29.7675109553675
5.2 29.7244268817888
5.3 29.6753278058147
5.4 29.6195799815382
5.5 29.557550475959
5.6 29.4910108395233
5.7 29.4247700284703
5.8 29.368753703617
5.9 29.3479431559394
6 29.362347959718
6.1 29.3872630615863
6.2 29.4128147925349
6.3 29.4343202938591
6.4 29.4466763930011
6.5 29.4501309888688
6.6 29.4468911180372
6.7 29.4436016931068
6.8 29.4525701382096
6.9 29.476731471043
7 29.5133332468865
7.1 29.5514918485651
7.2 29.5872164468915
7.3 29.6193129656351
7.4 29.6475743296381
7.5 29.672615786462
7.6 29.69485799826
7.7 29.7142582222253
7.8 29.7309225465103
7.9 29.7452886192518
8 29.7573878162699
8.1 29.7676053003733
8.2 29.7760351143719
8.3 29.7826915699602
8.4 29.7876476262833
8.5 29.7913215607711
8.6 29.7948272781314
8.7 29.7981932795367
8.8 29.8014628598351
8.9 29.8046757352642
9 29.8073486314913
9.1 29.8078978756643
9.2 29.8066487170961
9.3 29.8060705905689
9.4 29.8064307699101
9.5 29.8063451462254
9.6 29.806292987689
};
\addlegendentry{MHE}
\addplot [semithick, darkorange25512714]
table {%
0 29.3274998664856
0.1 29.3835258483887
0.2 29.3680119514465
0.3 29.4310474395752
0.4 29.7576451301575
0.5 29.7484564781189
0.6 29.7926449775696
0.7 29.7981643676758
0.8 29.6980094909668
0.9 29.878785610199
1 29.857165813446
1.1 29.9179172515869
1.2 29.9164223670959
1.3 29.9150323867798
1.4 33.3889579772949
1.5 33.2858777046204
1.6 33.3375978469849
1.7 33.3361768722534
1.8 33.3684635162354
1.9 30.2332973480225
2 30.2248215675354
2.1 30.2245020866394
2.2 30.1672410964966
2.3 30.1745629310608
2.4 28.722186088562
2.5 28.6648797988892
2.6 29.2821002006531
2.7 29.2743802070618
2.8 29.2877626419067
2.9 29.6547651290894
3 29.7553157806396
3.1 29.7611093521118
3.2 29.6592974662781
3.3 29.7596192359924
3.4 29.8017287254333
3.5 29.7646999359131
3.6 29.8072504997253
3.7 29.727566242218
3.8 29.7275638580322
3.9 30.2727627754211
4 30.3301358222961
4.1 30.3437399864197
4.2 30.4007601737976
4.3 30.4137873649597
4.4 30.2204084396362
4.5 30.1773428916931
4.6 30.2267575263977
4.7 30.1699662208557
4.8 30.2833962440491
4.9 30.2099585533142
5 30.2534770965576
5.1 30.2581000328064
5.2 30.3284239768982
5.3 30.3348684310913
5.4 30.4528188705444
5.5 30.3926706314087
5.6 30.3166913986206
5.7 29.9616432189941
5.8 29.9082136154175
5.9 23.3457112312317
6 23.3594369888306
6.1 29.7974634170532
6.2 29.8414921760559
6.3 29.776623249054
6.4 30.8763122558594
6.5 30.5327796936035
6.6 30.5541181564331
6.7 30.0142312049866
6.8 27.2695922851562
6.9 27.3576164245605
7 27.4155187606812
7.1 30.045690536499
7.2 30.0785350799561
7.3 30.045530796051
7.4 30.0823950767517
7.5 29.9367904663086
7.6 29.8991060256958
7.7 29.9858689308167
7.8 30.0239253044128
7.9 29.9223399162292
8 30.0128126144409
8.1 29.9160695075989
8.2 29.9366140365601
8.3 29.9555039405823
8.4 29.9850034713745
8.5 29.9849247932434
8.6 29.7009897232056
8.7 29.8046278953552
8.8 29.8136830329895
8.9 29.7589874267578
9 29.7533893585205
9.1 30.2161741256714
9.2 30.2082896232605
9.3 29.5168232917786
9.4 29.5461106300354
9.5 30.0358963012695
9.6 30.0358867645264
};
\addlegendentry{Naive}
\end{axis}

\end{tikzpicture}


==> sections/EXPERIMENTS/strategy_for_training_long_range.tex <==
\subsection{Strategies for Training Long Range Detector}   \label{subsec:range_thresh_and_wt}

\input{tables/Ablation_range_thresholding}

The effect of range threshold and range weighing on the \gls{fsd} trained using \gls{mvp} is summarised in~\Cref{tab:range_ablation}. The general experts are optimised to target objects in the full 0-250~\si{m} range while the long- (mid-) range experts aim to maximise the performance for distances $>$ ($\leq$) 100~\si{m}. 
~\Cref{table:range_wts} further denotes the range weights for both mid and long range experts for different values of range thresholding $r_1$ and $r_2$. These weights are computed using \cref{eq:weights} together with the the bin-wise label statistics of the training set, which were shown in \cref{fig:Statistics_dataset}.


%Given the large difference in the number of labeled objects as a function of their distance, which was illustrated in \cref{fig:Statistics_dataset}, it is only natural that the FSD$_{0-250}$ algorithm, which is used as baseline in this experiment, performs best for near objects within distances below 50 m. In order to improve performance on long range points, two different approaches are tested: range thresholding and range weighing. The former consists on training the algorithm using only a subset of objects with a specific distance we are aiming to target. The latter consists on reducing the imbalance of labeled objects between distances by increasing the impact on the loss function on objects that are further away. 


\input{tables/Method_range_weighing_values}

The range weights, which are implemented in FSD$_{0-250}^{w}$, show a performance improvement in the 50-150~\si{m} range with respect to FSD$_{0-250}$ and a performance degrading in the below 50~\si{m} range. We also train long-range experts using range thresholding of $50-250$~\si{m} and $100-250$~\si{m} with and without range weights for comparison. In particular, FSD$_{100-250}$ corresponds to simply finetuning the network for long-range points, and it performs the worst in 100-150~\si{m} range. It is observed that range weighing leads to slight improvements for both long-range experts. Moreover, it is found that the best performance for a range bin $b$ can be obtained by using range thresholding from bin $b-1$ in combination with range weighing i.e. the best performance at $100-150$~\si{m} is obtained by FSD$_{50-250}^{w}$. We also train a short range expert, referred as FSD$_{0-100}$, using range thresholding of $0-100$~\si{m}. Range weights are not applied in this case in order not to degrade the performance at $0-50$~\si{m}. As expected, the short range expert results in the most optimal performance for objects at $0-50$~\si{m}, while the performance at  $50-100$~\si{m} is only degraded by 0.1\% with respect to FSD$_{0-250}^{w}$. Based on the results, we choose FSD$_{0-100}$ and FSD$_{50-250}^{w}$ as the mid- and long- range experts, and merge them to form RangeFSD, a network with high performance at both mid and long range.


%The range weights, which are implemented in FSD$_{0-250}^{w}$, show a performance improvement in the range 50-150 range with respect to FSD$_{0-250}$ and a performance degrading in the below 50 m range. Long range experts are trained using range thresholding of $50-250$ and $100-250$ with and without range weights in order to improve the performance of objects at long range. The best performance for far away objects in the $100-200$ range is found when combining both approaches. In particular, it is found that the best performance for a range bin $n$ can be obtained by using range thresholding from bin $n-1$ in combination with range weighing i.e. the best performance at $100-150$ is obtained by FSD$_{50-250}^{w}$, while the best performance at  $150-200$  is obtained by FSD$_{100-250}^{w}$. A short range expert, referred as FSD$_{0-100}$, is also trained using range thresholding of $0-100$. Range weights are not applied in this case in order to not degrade the performance at $0-50$ m. As expected, the short range expert results in the most optimal performance for objects at $0-50$ m, while the performance at  $50-100$ m is only degraded by 0.1 with respect to FSD$_{0-250}^{w}$, which yields the best performance for that range. The mid- and long- range experts, FSD$_{0-100}$ and FSD$_{50-250}^{w}$, are merged to form RangeFSD, a network with high performance at both mid and long range.


==> sections/limitations.tex <==
% Three notable limitations of our proposed method merit discussion. 
\section{Limitations} \label{sec:limitations}

==> tikz/1D532054-768E-486D-BA06-30FB3C390865.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={time},
xmajorgrids,
xmin=0, xmax=10,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Speed (m/s)},
ymajorgrids,
ymin=0, ymax=40,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0 6.71202471234191
0.1 6.71212650413523
0.2 6.71320161601858
0.3 6.71571971145201
0.4 6.72183766613334
0.5 6.73019302157916
0.6 6.73637694780359
0.7 6.72831439055839
0.8 6.71658761051972
0.9 6.70353010039088
1 6.6863083361169
1.1 6.66520356688714
1.2 6.6440739385626
1.3 6.62353394143528
1.4 6.6017390364367
1.5 6.57822516287673
1.6 6.55181858610996
1.7 6.5219881844951
1.8 6.48901217213124
1.9 6.45498217609582
2 6.42040472652682
2.1 6.38526597797995
2.2 6.34992393769454
2.3 6.31412754569929
2.4 6.27744069368862
2.5 6.24047579420392
2.6 6.20405040538093
2.7 6.16831099291595
2.8 6.13411080999295
2.9 6.1026085199839
3 6.07311337720809
3.1 6.04354817574024
3.2 6.01410066576357
3.3 5.98582675756972
3.4 5.96039648180083
3.5 5.93806514067297
3.6 5.91911989930222
3.7 5.90475938790188
3.8 5.89680292266841
3.9 5.89657942828985
4 5.90445939137127
4.1 5.92026693720539
4.2 5.94128418761199
4.3 5.96563960412441
4.4 5.99103220459708
4.5 6.01673836495861
4.6 6.04336436986499
4.7 6.07123543054912
4.8 6.10108892359348
4.9 6.13269345316793
5 6.16502124783009
5.1 6.19818676420169
5.2 6.23143479438893
5.3 6.26512614059627
5.4 6.29889951798765
5.5 6.33149212548943
5.6 6.36319048658953
5.7 6.3941031046647
5.8 6.42466041855346
5.9 6.45407135865259
6 6.48203266028448
6.1 6.50831679308746
6.2 6.53295258396727
6.3 6.55656184321725
6.4 6.57919820833863
6.5 6.6028206709945
6.6 6.62858816637784
6.7 6.65684960347955
6.8 6.68759273171915
6.9 6.72078231273906
7 6.75635494153552
7.1 6.79435742714861
7.2 6.83354901874738
7.3 6.87346262441178
7.4 6.91390608843172
7.5 6.95462994766928
7.6 6.99505008793036
7.7 7.03345227754504
7.8 7.06504824964518
7.9 7.08821522010447
8 7.10257934442056
8.1 7.10862388162113
8.2 7.10856420733003
8.3 7.10853153423777
};
\addlegendentry{MHE}
\addplot [semithick, darkorange25512714]
table {%
0 6.50924695475223
0.1 6.77862505903709
0.2 6.57466667111938
0.3 6.73709675686949
0.4 6.00555144567131
0.5 6.18860032793027
0.6 6.19155846094841
0.7 10.4031983765258
0.8 6.28092210486421
0.9 6.29285667271901
1 7.40369869457888
1.1 7.42492895200204
1.2 6.3447902097414
1.3 6.35252199190382
1.4 6.9063558320403
1.5 6.72180178408042
1.6 6.94588659326776
1.7 6.97126227138414
1.8 7.00301521405625
1.9 6.43704061691167
2 6.46731306302387
2.1 6.50809036336751
2.2 6.33841326911777
2.3 6.37447281182024
2.4 6.49167319867468
2.5 6.31905883012231
2.6 6.13093823637765
2.7 6.20854166157762
2.8 6.04958433796676
2.9 5.6823597438689
3 5.74522187628929
3.1 6.2978029289496
3.2 6.11672020503744
3.3 5.95702334340392
3.4 5.57851957383552
3.5 5.66322777366265
3.6 5.69505841771691
3.7 5.52870104860443
3.8 5.20742053071722
3.9 5.03235669975401
4 5.03533632683853
4.1 4.86202752806491
4.2 5.49694352765755
4.3 5.56715262362991
4.4 6.03194432026411
4.5 6.09996080477162
4.6 5.90382291269483
4.7 5.96854085522395
4.8 5.77286240968193
4.9 5.84912304273175
5 6.17001890434511
5.1 5.99934653557052
5.2 6.30827714112921
5.3 6.12178191947726
5.4 6.17354025451713
5.5 6.56666000579845
5.6 6.40003574507065
5.7 6.46327933457758
5.8 6.30537084236629
5.9 6.58478096363733
6 6.60807294110667
6.1 6.675068428527
6.2 6.72940990446505
6.3 6.57634495339401
6.4 6.83851640014947
6.5 6.3985883750721
6.6 6.30040362364653
6.7 6.33987820909524
6.8 6.39914758423188
6.9 6.43878886541034
7 6.49241253530109
7.1 6.38845069281766
7.2 6.75455174956129
7.3 6.78998577595216
7.4 6.81123091701026
7.5 6.84662511636138
7.6 6.86786527920537
7.7 6.88916615650134
7.8 8.03334067848102
7.9 8.03619033996073
8 8.05843708869443
8.1 8.10888080106935
8.2 8.1132128096501
8.3 8.15288156239514
};
\addlegendentry{Naive}
\end{axis}

\end{tikzpicture}

